Geometric L1 Adaptive Attitude Control for a Quadrotor Unmanned Aerial Vehicle

In this paper, we study the quadrotor UAV attitude control on SO(3) in the presence of unknown disturbances and model uncertainties. L1 adaptive control for UAVs using Euler angles/quaternions is shown to exhibit robustness and precise attitude tracking in the presence of disturbances and uncertainties. However, it is well known that dynamical models and controllers that use Euler angle representations are prone to singularities and typically have smaller regions of attraction while quaternion representations are subject to the unwinding phenomenon. To avoid such complexities, we present a Geometric L1 adaptation control law to estimate the uncertainties. A model reference adaptive control approach is implemented, with the attitude errors between the quadrotor model and the reference model defined on the manifold. Control laws for the quadrotor and reference models are developed directly on SO(3) to track the desired trajectory while rejecting the uncertainties. Control Lyapunov function based analysis is used to show the exponential input-to-state stability of the attitude errors. The proposed L1 adaptive controller is validated using numerical simulations. Preliminary experimental results are shown comparing a geometric PD controller to the geometric L1 adaptive controller. Experimental validation of the proposed controller is carried out on an Autel X-star quadrotor.

==> hover_metrics.tex <==
bl_mean_pos_err =

    0.0152


bl_var_pos_err =

   1.3864e-04


bl_sigma_pos_err =

    0.0118


bl_mean_vel_err =

    0.0359


bl_var_vel_err =

   8.5087e-04


bl_sigma_vel_err =

    0.0292


bl_mean_psi_err =

    0.0055


bl_var_psi_err =

    0.0021


bl_sigma_psi_err =

    0.0462


l1_mean_pos_err =

    0.0182


l1_var_pos_err =

   1.7400e-04


l1_sigma_pos_err =

    0.0132


l1_mean_vel_err =

    0.0435


l1_var_vel_err =

    0.0011


l1_sigma_vel_err =

    0.0337


l1_mean_psi_err =

    0.0021


l1_var_psi_err =

    0.0020


l1_sigma_psi_err =

    0.0452

==> l1_diag.tex <==
\definecolor{uuuuuu}{rgb}{0.26666666666666666,0.26666666666666666,0.26666666666666666}\definecolor{ffzzqq}{rgb}{1,0.6,0}\definecolor{wwccff}{rgb}{0.4,0.8,1}\definecolor{zzttqq}{rgb}{0.6,0.2,0}\definecolor{zzccff}{rgb}{0.6,0.8,1}\definecolor{ududff}{rgb}{0.30196078431372547,0.30196078431372547,1}\definecolor{cqcqcq}{rgb}{0.7529411764705882,0.7529411764705882,0.7529411764705882}\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]\draw [color=cqcqcq,, xstep=2cm,ystep=2cm] (-12.64219412154657,-14.01934660298175) grid (13.446446359108503,9.485971660393973);\draw[->,color=black] (-12.64219412154657,0) -- (13.446446359108503,0);\foreach \x in {-12,-10,-8,-6,-4,-2,2,4,6,8,10,12}\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {\footnotesize $\x$};\draw[->,color=black] (0,-14.01934660298175) -- (0,9.485971660393973);\foreach \y in {-14,-12,-10,-8,-6,-4,-2,2,4,6,8}\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {\footnotesize $\y$};\draw[color=black] (0pt,-10pt) node[right] {\footnotesize $0$};\clip(-12.64219412154657,-14.01934660298175) rectangle (13.446446359108503,9.485971660393973);\fill[line width=2pt,color=zzccff,fill=zzccff,fill opacity=0.33] (-10,8) -- (10,8) -- (10,2) -- (-10,2) -- cycle;\fill[line width=2pt,color=zzttqq,fill=zzttqq,fill opacity=0.10000000149011612] (-10,-2) -- (10,-2) -- (10,-8) -- (-10,-8) -- cycle;\fill[line width=2pt,color=wwccff,fill=wwccff,fill opacity=0.43] (-4,6) -- (4,6) -- (4,4) -- (-4,4) -- cycle;\fill[line width=2pt,color=zzttqq,fill=zzttqq,fill opacity=0.13] (4,-4) -- (4,-6) -- (-4,-6) -- (-4,-4) -- cycle;\fill[line width=2.8pt,color=ffzzqq,fill=ffzzqq,fill opacity=0.09] (-2,1) -- (2,1) -- (2,-1) -- (-2,-1) -- cycle;\draw [line width=2pt,color=zzccff] (-10,8)-- (10,8);\draw [line width=2pt,color=zzccff] (10,8)-- (10,2);\draw [line width=2pt,color=zzccff] (10,2)-- (-10,2);\draw [line width=2pt,color=zzccff] (-10,2)-- (-10,8);\draw [line width=2pt,color=zzttqq] (-10,-2)-- (10,-2);\draw [line width=2pt,color=zzttqq] (10,-2)-- (10,-8);\draw [line width=2pt,color=zzttqq] (10,-8)-- (-10,-8);\draw [line width=2pt,color=zzttqq] (-10,-8)-- (-10,-2);\draw [line width=2pt,color=wwccff] (-4,6)-- (4,6);\draw [line width=2pt,color=wwccff] (4,6)-- (4,4);\draw [line width=2pt,color=wwccff] (4,4)-- (-4,4);\draw [line width=2pt,color=wwccff] (-4,4)-- (-4,6);\draw [line width=2pt,color=zzttqq] (4,-4)-- (4,-6);\draw [line width=2pt,color=zzttqq] (4,-6)-- (-4,-6);\draw [line width=2pt,color=zzttqq] (-4,-6)-- (-4,-4);\draw [line width=2pt,color=zzttqq] (-4,-4)-- (4,-4);\draw (-1.8202395517933547,6.205069809075328) node[anchor=north west] {$\textsc{Robot\, Model}\\ \quad \dot{R}=R\Omega^{\times}\\ \acute{J}\dot{\Omega}=M-(\Omega^{\times}\acute{J}\Omega)$};\draw (-1.8443957003865539,-3.661070758104312) node[anchor=north west] {$\textsc{Reference\, Model}\\ \quad \dot{\hat{R}}=\hat{R}\hat{\Omega}^{\times}\\ {J}\dot{\hat{\Omega}}=\hat{M}-(\hat{\Omega}^{\times}{J}\hat{\Omega})$};\draw [line width=2.8pt,color=ffzzqq] (-2,1)-- (2,1);\draw [line width=2.8pt,color=ffzzqq] (2,1)-- (2,-1);\draw [line width=2.8pt,color=ffzzqq] (2,-1)-- (-2,-1);\draw [line width=2.8pt,color=ffzzqq] (-2,-1)-- (-2,1);\draw (-1.361272728522571,1.1431069527551327) node[anchor=north west] {$\textsc{\,\,\,\,Desired \,\\ Trajectory}\\ \quad R_d,\,\Omega_d$};\draw [->,line width=2.8pt] (0,1) -- (0,4);\draw [->,line width=2.8pt] (0,-1) -- (0,-4);\begin{scriptsize}\draw [fill=ududff] (-10,10) circle (2.5pt);\draw[color=ududff] (-12.545569527173773,9.755474312466577) node {$A$};\draw [fill=ududff] (10,10) circle (2.5pt);\draw[color=ududff] (-12.545569527173773,9.755474312466577) node {$B$};\draw [fill=ududff] (10,4) circle (2.5pt);\draw[color=ududff] (10.185366299026619,4.506031350356744) node {$C$};\draw [fill=ududff] (-10,4) circle (2.5pt);\draw[color=ududff] (-9.81592473614227,4.506031350356744) node {$D$};\draw [fill=ududff] (-10,2) circle (2.5pt);\draw[color=ududff] (-9.81592473614227,2.5140552263418523) node {$E$};\draw [fill=ududff] (10,2) circle (2.5pt);\draw[color=ududff] (10.185366299026619,2.5140552263418523) node {$F$};\draw [fill=ududff] (10,8) circle (2.5pt);\draw[color=ududff] (10.185366299026619,8.513418611610232) node {$G$};\draw [fill=ududff] (-10,8) circle (2.5pt);\draw[color=ududff] (-9.81592473614227,8.513418611610232) node {$H$};\draw [fill=ududff] (-10,-2) circle (2.5pt);\draw[color=ududff] (-9.81592473614227,-1.4933320349116357) node {$I$};\draw [fill=ududff] (10,-2) circle (2.5pt);\draw[color=ududff] (10.185366299026619,-1.4933320349116357) node {$J$};\draw [fill=ududff] (10,-8) circle (2.5pt);\draw[color=ududff] (10.185366299026619,-7.4926954201800156) node {$K$};\draw [fill=ududff] (-10,-8) circle (2.5pt);\draw[color=ududff] (-9.81592473614227,-7.4926954201800156) node {$L$};\draw[color=zzccff] (0.08809618706937743,7.904108267793912) node {$h$};\draw[color=zzccff] (9.702243327162636,5.279386786738996) node {$g$};\draw[color=zzccff] (0.08809618706937743,2.65466530568408) node {$f$};\draw[color=zzccff] (-9.526050953023882,5.279386786738996) node {$e$};\draw[color=zzttqq] (0.08809618706937743,-2.1026423787279556) node {$i$};\draw[color=zzttqq] (9.702243327162636,-4.727363859782871) node {$j$};\draw[color=zzttqq] (0.08809618706937743,-7.352085340837788) node {$k$};\draw[color=zzttqq] (-9.526050953023882,-4.727363859782871) node {$l$};\draw [fill=ududff] (-4,6) circle (2.5pt);\draw[color=ududff] (-3.8010437364356844,6.498007474371636) node {$M$};\draw [fill=ududff] (4,6) circle (2.5pt);\draw[color=ududff] (4.194641447913232,6.498007474371636) node {$N$};\draw [fill=ududff] (4,4) circle (2.5pt);\draw[color=ududff] (4.194641447913232,4.506031350356744) node {$O$};\draw [fill=ududff] (-4,4) circle (2.5pt);\draw[color=ududff] (-3.8010437364356844,4.506031350356744) node {$P$};\draw [fill=ududff] (-4,-4) circle (2.5pt);\draw[color=ududff] (-3.8010437364356844,-3.4853081589265273) node {$Q$};\draw [fill=ududff] (4,-4) circle (2.5pt);\draw[color=ududff] (4.194641447913232,-3.4853081589265273) node {$R$};\draw [fill=ududff] (4,-6) circle (2.5pt);\draw[color=ududff] (4.194641447913232,-5.500719296165124) node {$S$};\draw [fill=ududff] (-4,-6) circle (2.5pt);\draw[color=ududff] (-3.8010437364356844,-5.500719296165124) node {$T$};\draw[color=wwccff] (0.184720781442174,5.279386786738996) node {q3};\draw[color=wwccff] (0.08809618706937743,5.91213214377902) node {$m$};\draw[color=wwccff] (3.6873623274560496,5.279386786738996) node {$n$};\draw[color=wwccff] (0.08809618706937743,4.646641429698971) node {$o$};\draw[color=wwccff] (-3.535326101910494,5.279386786738996) node {$p$};\draw[color=zzttqq] (3.6873623274560496,-4.727363859782871) node {$r$};\draw[color=zzttqq] (0.08809618706937743,-5.336674203599191) node {$s$};\draw[color=zzttqq] (-3.535326101910494,-4.727363859782871) node {$t$};\draw[color=zzttqq] (0.08809618706937743,-4.094618502742847) node {$q$};\draw [fill=ududff] (-2,1) circle (2.5pt);\draw[color=ududff] (-1.7960834032001556,1.5063496577225541) node {$U$};\draw [fill=ududff] (2,1) circle (2.5pt);\draw[color=ududff] (0.3055015244081697,1.1079544329195758) node {$V$};\draw [fill=ududff] (2,-1) circle (2.5pt);\draw[color=ududff] (2.1896811146777027,-0.4856264662923376) node {$W$};\draw [fill=ududff] (-2,-1) circle (2.5pt);\draw[color=ududff] (-1.7960834032001556,-0.4856264662923376) node {$Z$};\draw[color=ffzzqq] (0.08809618706937743,0.8970393139062343) node {$u$};\draw[color=ffzzqq] (1.70655814281372,0.2877289700899145) node {$v$};\draw[color=ffzzqq] (0.08809618706937743,-0.3450163869501099) node {$w$};\draw[color=ffzzqq] (-1.4578973228953676,0.35803400976102834) node {$z_1$};\draw [fill=uuuuuu] (0,4) circle (2pt);\draw[color=uuuuuu] (0.2571892272217714,4.529466363580449) node {$A_1$};\draw [fill=uuuuuu] (0,1) circle (2pt);\draw[color=uuuuuu] (0.2571892272217714,1.5297846709462588) node {$B_1$};\draw [fill=uuuuuu] (0,-1) circle (2pt);\draw[color=uuuuuu] (0.2571892272217714,-0.46219145306863296) node {$C_1$};\draw [fill=uuuuuu] (0,-4) circle (2pt);\draw[color=uuuuuu] (0.2571892272217714,-3.4618731457028225) node {$D_1$};\draw[color=black] (-0.03268455589661827,2.771840371802603) node {$a$};\draw[color=black] (0.20887693003537314,-2.2198174448464782) node {$b$};\end{scriptsize}\end{tikzpicture}

==> l1scheme.tex <==
\section{$L_1$ Scheme}

%\begin{figure*}
%\centering
%\includegraphics[width=1.85\columnwidth]{l1_2}
%\label{fig:l1scheme}
%\caption{$L_1$ Adaptive scheme. {\color{red} Place holder for l1 schematic, needs to be updated}}
%\end{figure*}




==> perturbations.tex <==
\section{Mathematical Background}
\editWu{I will revise this section once I am done with it }
\subsection{Singular Perturbations}
\label{section:perturbations}
A standard {\it singular perturbation model} {\color{red} Tikhonov's theorem [CITE]} for a dynamical system is given by the following model \cite{khalil1996nonlinear},
\begin{equation}
\label{eq:sing1}
\dot{x} = f(t,x,z,\varepsilon),
\end{equation}
\begin{equation}
\label{eq:sing2}
\varepsilon \dot{z} = g(t,x,z,\varepsilon),
\end{equation}
where $x$ and $z$ are two different set of system states and $f$ and $g$ are continously differentiable with respect to their arguments $t$, $x$, $z$ and $\varepsilon$. Domain for the given system is given as,
\begin{equation*}
(t,x,z,\varepsilon) \in [0,t_1]\times D_x \times D_z \times [0,\varepsilon_0],
\end{equation*}
where $D_x \subset \mathbb{R}^n$ and $D_z \subset \mathbb{R}^m$ are open connected sets and $t_1\in \mathbb{R}$, $\varepsilon_0 \in \mathbb{R}$. 

Setting $\varepsilon=0$, results \eqref{eq:sing2} into the following algebraic equation,
\begin{equation}
\label{eq:sing3}
0 = g(t,x,z,\varepsilon).
\end{equation} 

The dynamics of the system, \eqref{eq:sing1}, \eqref{eq:sing2} degenerates into the dynamics given in \eqref{eq:sing1} and the algebraic equation \eqref{eq:sing3}. Dimension of the system reduces from $n+m$ to $n$. The positive real roots for \eqref{eq:sing3} can be expressed as,
\begin{equation}
z = h_i(t,x),\quad i=1,2,\hdots,k,\quad k\geq 1,
\end{equation}
for $t\in [0,t1]$ and $x\in D_x$. Dynamics of the system corresponding to a well-defined root $h_i$ is,
\begin{equation}
\label{eq:sing4}
\dot{x} = f(t,x,h_i(t,x),0).
\end{equation}
	
We have $\dot{z} = g/\varepsilon$ from \eqref{eq:sing2}, thus, having a very small $\varepsilon$ tending to zero, results in a very high value for $\dot{z}$, for $g\neq 0$, implying that the system may converge to the roots of \eqref{eq:sing3} rapidly. As stated in \cite{khalil1996nonlinear}, the dynamics given in \eqref{eq:sing4} is called {\it the slow model}. 

{\color{red} have to write a connecting paragraph}
Performing a change of variable, with $y = z-h(t,x)$, scaling the time $t$, such that we get a new variable $\tau = \frac{t-t_)}{\varepsilon}$, where $t_0$ is the initial time and setting the value of $\varepsilon$ to zero, we get, 
\begin{equation}
\label{eq:boundary}
\frac{\partial y}{\partial \tau} = g(t,x,y+h(t,x),0),
\end{equation}
where $(t,x)\in [0,t_1]\times D_x$ is constant w.r.t. $\tau$. This above equation is refered to as boundary layer system. 

{\color{red} the following paragraph is exactly copied from Khalil book}
\begin{thm}
\label{thm1}
Singular perturbation model,
\begin{equation}
\dot{x} = f(t,x,z,\varepsilon),\quad x(t_0)=\xi(\varepsilon),
\end{equation}
\begin{equation}
\varepsilon\dot{z} = g(t,x,z,\varepsilon),\quad z(t_0)=\eta(\varepsilon),
\end{equation}
where, the initial conditions for $x(t_0)$ and $z(t_0)$ are smooth functions of $\varepsilon$ given by $\xi(\varepsilon)$ and $\eta(\varepsilon)$ respectively. Let $z = h(t,x)$ be an isolated root of \eqref{eq:sing3}. We assume that the following conditions are satisfied for all,
\begin{equation*}
[t,x,z-h(t,x),\varepsilon]\in [0,\infty)\times D_x \times D_y \times [0,\varepsilon_0]
\end{equation*}
for some domains $D_x \subset \mathbb{R}^n$ and $D_y\subset \mathbb{R}^m$, which contain their origins:
\begin{itemize}
\item On an compact subset of $D_x\times D_y$, the functions f, g, their first partial derivatives with respect to $(x, z, \varepsilon)$, and the first partial derivative of with respect to $t$ are continous and bounded. $h(t,x)$ and $[\partial g(t,x,z,0)/\partial z]$ have bounded first partial derivatives with respect to their arguments, and $[\partial f(t,x,h(t,x),0)/\partial x]$ is Lipschitz in $x$, uniformly in t;
 
\item the origin is an exponentially stable equilibrium point of the reduced system \eqref{eq:sing4}; there is a Lyapunov function $V(t,x)$ that satisfies the conditions of a exponential stable function for $(t,x)\in[0,\infty)\times D_x$ and $\{W_1(x)\leq c\}$ is a compact subset of $D_x$;

\item the origin is an exponentially stable equilibrium point of the boundary-layer system \eqref{eq:boundary}, uniformly in (t,x); let $R_y \subset D_y$ be the region of attraction of $\partial y/\partial \tau = g(t,x,y+h(t,x),0)$ and $\Omega_x$ be compact subset of $R_y$.
\end{itemize}

Then, for each compact set $\Omega_x\subset \{W_2(x) \leq \rho c, 0\leq \rho <1\}$ there is a positive constant $\varepsilon^*$ such that for all $t_0\geq 0$, $\xi_0 \in \Omega_x$, $\eta_0 - h(t_0,\xi_0)\in \Omega_y$, and $0<\varepsilon<\varepsilon*$, the singular perturbations model has a unique solution $x(t,\varepsilon)$, $z(t,\varepsilon)$ on $[t_0, \infty)$, and 
\begin{equation}
x(t,\varepsilon) - \bar{x}(t) = O(\varepsilon)
\end{equation}
\begin{equation}
z(t,\varepsilon) - h(t,\bar{x}(t)) - \hat{y}(t/\varepsilon) = O(\varepsilon)
\end{equation}
hold uniformly for $t\in [t_0, \infty)$, where $\bar{x}(t)$ and $\hat{y}(\tau)$ are the solutions of the reduced and boundary-layer problems 
\begin{equation*}
\dot{x} = f(t,x,h(t,x),0),\quad x(t_0)=\xi_0 \equiv	\xi(0)
\end{equation*}
and
\begin{equation*}
\frac{\partial y}{\partial \tau} = g(t_0,\xi_0, y+h(t_0,\xi_0),0),\quad y(0) = \eta(0)-h(t_0,\xi_0).
\end{equation*}
Moreover, given $t_b > t_0$, there is $\varepsilon^{**}\leq \varepsilon^*$ such that
\begin{equation}
z(t,\varepsilon)-h(t,\bar{x}(t)) = O(\varepsilon)
\end{equation}
holds uniformly for $t\in [t_b,\infty)$ whenever $\varepsilon < \varepsilon^{**}$.
\end{thm}

Proof for the above theorem is given in \cite{khalil1996nonlinear}. 








